Evaluating and Optimizing Hearing-Aid Self-Fitting Methods using Population Coverage

Adults with mild-to-moderate hearing loss can use over-the-counter hearing aids to treat their hearing loss at a fraction of traditional hearing care costs. These products incorporate self-fitting methods that allow end-users to configure their hearing aids without the help of an audiologist. A self-fitting method helps users configure the gain-frequency responses that control the amplification for each frequency band of the incoming sound. This paper considers how to design effective self-fitting methods and whether we may evaluate certain aspects of their design without resorting to expensive user studies. Most existing fitting methods provide various user interfaces to allow users to select a configuration from a predetermined set of presets. We propose a novel metric for evaluating the performance of preset-based approaches by computing their population coverage. The population coverage estimates the fraction of users for which it is possible to find a configuration they prefer. A unique aspect of our approach is a probabilistic model that captures how a user's unique preferences differ from other users with similar hearing loss. Next, we develop methods for determining presets to maximize population coverage. Exploratory results demonstrate that the proposed algorithms can effectively select a small number of presets that provide higher population coverage than clustering-based approaches. Moreover, we may use our algorithms to configure the number of increments for slider-based methods.

==> approach.tex <==
\section{Approach}
\label{sec:approach}

% \input{problem-formulation}
% \input{data-characteristics}
% \input{greedy_algorithm}
% \input{genetic_algorithm}


==> bullets.tex <==
- Issues with previous method (Clustering & Coverage)
    - Issues with clustering
        - Not uniformly distributed
        - Clumps in the center where population weight is higher
    - Issues with coverage criteria (+- 5 dB within NAL-NL2)
        - 50% of participants in a previous study preferred more than +- 5 dB presets
        - This observation motivates the need for new coverage criteria
        
- Defining new coverage criteria
    - Defining transfer function
    - Rationale for using specific shapes
    - Defining variations
    - Defining variation weights
    - Rationale for using previous studies to generate weights
    - Defining new coverage (80% of variation weights / +- 5 dB covered)
    
- Rationale for using REAR vs REIG
    - From audiologist (From our discussion, there was no clear consensus)

- Rationale for using additional NHANES points
    - To cover more population with mild-to-moderate sensorineural hearing loss
    
- Problem formulation
    - Define the problem mathematically
   
- Heuristic methods for preset generation
    - Genetic Algorithm
    - Algorithm's working
    - Algorithm's pseudo-code

- Defining other self-fitting methods (Optional)
    - 2 Param method
    - PCA method
    - Goldilocks method
    
- Optimizing other methods (Optional)
    - Details about optimizing other self-fitting methods for coverage
    
- Comparison & Discussion
    - Comparisons between different subgroups and their performances in terms of coverage
    - Discussion

==> data-characteristics.tex <==
\subsection{Data Characteristics}

As discussed in Section \ref{subsec:reig-target-generation}, we used the NHANES dataset to derive 4418 REIGs that represent the US Population with mild-to-moderate hearing loss.
In this paper, we considered REIG levels across 6 different frequencies (0.5, 1, 2, 3, 4, 6 kHz) at 65 dB SPL.
Figure \ref{fig:reig-boxplots} shows gain ranges across all the frequencies.

\Figure[t!](topskip=0pt, botskip=0pt, midskip=0pt)[scale=0.5]{Figures/reig_boxplots.pdf}
{REIG distribution of NHANES Data. \label{fig:reig-boxplots}}

As discussed in Section \ref{subsec:transfer-function-development}, we have 357,858 total variations from which to choose a limited number of presets that maximize the population coverage according to our defined coverage criteria.
Due to this large search space, it would be difficulty for a HA user to arrive at their optimal gain-frequency response. 
We propose two solutions to reduce the search space.
First, we propose using dimensionality reduction using PCA to reduce REIG dimensions to 2.
Second, instead of considering the entire continuous space across 2-dimensions, we discretize the feature space.
Figure \ref{fig:pca-plot-reig} shows PCA plot of the 4418 REIG data points in PCA space.
Figure \ref{fig:pca-plot-variations} shows 357858 variation points in PCA space. 
Figure \ref{fig:pca-plot-combined} shows both original REIG points and variations.
It can be noted that the search space increases significantly after using transfer functions to create variation REIG points.
In all cases, white contours depicts the density of data points.
In this case, PCA feature 1 corresponds to overall loudness and PCA feature 2 corresponds to spectral tilt.
This observation can be seen in Figure \ref{fig:reig-features}.


\Figure[t!](topskip=0pt, botskip=0pt, midskip=0pt)[scale=0.5]{Figures/pca_feature_effects_in_original_space.pdf}
{PCA features and its effects in original REIG space. \label{fig:reig-features}}

Next, we propose two different algorithms -- the Greedy algorithm and the Genetic algorithm -- to derive presets that maximize the population coverage given preset number constraints.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.95\linewidth]{Figures/datapoints_PCA_png.png}
%     \caption{PCA Plot of all the variations}
%     \label{fig:pca-plot-variations}
% \end{figure}

% \Figure[t!](topskip=0pt, botskip=0pt, midskip=0pt)[scale=0.5]{Figures/reig_points_PCA_png.png}
% {PCA Plot of NHANES REIGs. \label{fig:pca-plot-reig}}


% \Figure[t!](topskip=0pt, botskip=0pt, midskip=0pt)[scale=0.5]{Figures/datapoints_PCA_png.png}
% {PCA Plot of all the variations. \label{fig:pca-plot-variations}}

\begin{figure*} % for sub figures over two columns in 
\centering
\subfloat[Population Configs]{\includegraphics[width=0.32\linewidth]{Figures/reig_points_PCA_png.png} \label{fig:pca-plot-reig}}
\hfil
\subfloat[Variation Configs]{\includegraphics[width=0.32\linewidth]{Figures/datapoints_PCA_png.png} \label{fig:pca-plot-variations}}
\hfil
\subfloat[Combined Configs]{\includegraphics[width=0.32\linewidth]{Figures/datapoints_PCA_combined_png.png} \label{fig:pca-plot-combined}}
\caption{{Representation of NHANES configs, variations configs and Combined configs in PCA space}}
\label{fig:pca-plots-reig-variations-combined}
\end{figure*}


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.95\linewidth]{Figures/reig_boxplots.pdf}
%     \caption{REIG Boxplots of NHANES Data}
%     \label{fig:reig-boxplots}
% \end{figure}

% \Figure[t!](topskip=0pt, botskip=0pt, midskip=0pt)[scale=0.5]{Figures/reig_boxplots.pdf}
% {REIG Boxplots of NHANES Data. \label{fig:reig-boxplots}}


==> genetic_algorithm.tex <==
\subsection{Genetic Algorithm}
\label{subsec:genetic-algorithm}

In this subsection, we will explain how a Genetic Algorithm (GA) as a heuristic method can be applied to preset generation problem.
Pseudocode for the algorithm can be seen in Algorithm \ref{alg:genetic-algorithm}.

At a high level, we performed similar first few steps as we did in the greedy algorithm by discritizing PCA space and precomputing the coverage of each of the discrete points.
We randomly initialized a set of preset pools $PP$.
We computed fitness score (i.e., population coverage) of each these preset sets from $PP$.
We performed local improvements on the preset sets in $PP$.
We then generated a newer population by using a crossover technique on the presets within the preset pool $PP$.
We created a new set of preset sets $PP$ by including newly generated population and top half population in next iteration of improvement.
We repeated this step until we arrived at the maximum number of iteration allowed.
We then used Equation \ref{eq:maximize-coverage} to output the best performing preset set from $PP$.

% \subsubsection{Algorithm Outline}
% \begin{itemize}
%     \item Divide PCA space in discrete space (variables: step\_size) 
%     \item Precompute each points coverage
%     \item Start with random 250 pairs with number of clusters (ie, 20, 25, 30 etc.)
%     \item Iterate through each pairs until max\_iterations are reached (in our case: 500)
%     \begin{itemize}
%         \item Find each combination's fitness score (population coverage)
%         \item Perform local improvement on top 5 individuals with best fitness score
%         \item Create new population by crossover between top half of the population
%     \end{itemize}
%     \item Output the best performing pair with the highest fitness score
% \end{itemize}

\begin{algorithm}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwRepeat{Do}{do}{while}%
    % \underline{function Euclid} $(a,b)$\;
    \Input{$preset\_number, step\_size$, $max\_iterations$}
    \State Discritize PCA space by $step\_size$ in each dimension \\
    \State Precompute population coverage by each discrete point in PCA space \\
    \State $iterations \leftarrow 0$ \\
    \State Initialize $PP$ by randomly generating 250 pairs of preset set of size $preset\_number$ \\
    \While{iterations <= max\_iterations}{
        \State Compute fitness score of each $P \in PP$ using Equation \ref{eq:preset-set-coverage}\\
        \State Perform local improvements for each $P \in PP$ \\
        \State Create new population by using crossover technique between top half of the population for all preset sets in $PP$\\
        \State $iterations \leftarrow iterations + 1$
        }
    \Output{P_{max} = argmax_{P \in PP} PC(P)}
    \caption{Genetic algorithm for preset generation}
    \label{alg:genetic-algorithm}
\end{algorithm}


==> greedy_algorithm.tex <==
\subsection{Greedy Algorithm}
\label{subsec:greedy-algorithm}

In this subsection, we will explain how a greedy algorithm can be applied to preset generation problem for optimizing coverage.
Pseudocode for greedy algorithm can be found in Algorithm \ref{alg:greedy-algorithm}.

Briefly, we utilized dimensionality reduction and discritizing PCA space to reduce thousands of candidate REIG to hundreds.
We then precomputed population coverage by each of these discrete points in PCA space.
We greedily keep adding points with maximum population coverage until we get to the maximum allowed preset number constraint.
We use Equation \ref{eq:preset-set-coverage} to compute the population coverage of the output $P$.

% \subsubsection{Algorithm Outline}
% \begin{itemize}
%     \item Divide PCA space in discrete space (variables: step\_size) 
%     \item Precompute each points coverage
%     \item n = no of presets
%     \item P = $ \emptyset $
%     \item while(n > 0)
%     \begin{itemize}
%           \item Find the best preset $p_{max}$ with max coverage
%           \item P = $P \cup \{p_{max}\}$
%           \item Remove all the covered points from pre-computed coverage set
%           \item n = n - 1
%     \end{itemize}      
%     \item Output: P
% \end{itemize}

\begin{algorithm}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwRepeat{Do}{do}{while}%
    % \underline{function Euclid} $(a,b)$\;
    \Input{$preset\_number, step\_size$}
    \State Discritize PCA space by $step\_size$ in each dimension \\
    \State Precompute population coverage by each discrete point in PCA space \\
    \State $n \leftarrow preset\_number$ \\
    \State $P \leftarrow \emptyset$ \\
    \While{n > 0}{
        \State Find the best preset $p_{max}$ with the highest population coverage \\
        \State  $P = P \cup \{p_{max}\}$ \\
        \State Update the precomputed coverage by removing all the covered points by $p_{max}$ \\
        \State $n \leftarrow n - 1$
        }
    \Output{$P$}
    \caption{Greedy algorithm for preset generation}
    \label{alg:greedy-algorithm}
\end{algorithm}

==> notes.tex <==
% This tex document can be used for notes

% Mathematical definitions of transfer functions and variations.

% Given 

==> problem-formulation.tex <==
\subsection{Problem Formulation}
\label{subsec:problem-formulation}

We are given $n$ number of $d$ dimensional HA gain frequency responses (REIG) set $C = \{c_{1}, c_{2},...,c_{n}\}$, where $|c_{i}| = d, c_{i,j} \in R$.
We are also given $n$ number of population weights set $PW = \{pw_{1},pw_{2},...,pw_{n}\}, pw_{i} \in [0, 1], \sum_{i=1}^{n} pw_{i} = 1$ which corresponds to population weight of a corresponding REIG.
We are given a transfer function set $TF$ of $m$ length, such that $TF=\{tf_{1},tf_{2},...,tf_{m}\}$, where $|tf_{i}| = d, tf_{i,j} \in R$.
Further, we are given a variation weight set $TW$ of $m$ length, such that $TW = \{tw_{1},tw_{2},...,tw_{m}\}, tw_{i} \in [0, 1], \sum_{i=1}^{m} tw_{i} = 1$.
This transfer function set $TF$ is used to generate possible variations in elements of $C$.
The corresponding variation weight set, $TW$ is the likelihood of a variation being a preferred variation by the user (as discussed in Section \ref{subsec:transfer-function-development}).
Given these sets, we compute the preset variation set $CV = \{cv_{1}, cv_{2}, ... ,cv_{n}\}$, $|cv_{i}| = m, |cv_{i,j}| = d, cv_{i,j} = c_{i} \oplus tf_{j}$.

% oplus is element wise addition
% https://math.stackexchange.com/a/601545/376209

Given the maximum number of allowed presets $k$, our aim is to find a preset set $P$ such that $|P| \leq k, |p_{i}| = d, p_{i,j} \in R$ to maximize the population coverage by $P$.

Population coverage is computed by given $P$, $CV$ and threshold $th \in [0, 1]$ by following.

$y_{i,j} = 1, if \exists p \in P, s.t. max \{abs(x)  | x \in (p \ominus cv_{i,j})\} \leq 5$ else 0.
In short, $y_{i,j} = 1$ if any member in $P$ covers variation $cv_{i,j}$ i.e., one of the variations of $c_{i}$.

$y_{i} = 1, if \sum_{j=1}^{m} vw_{j} * y_{i,j} \ge th$ else 0.

Based on these values, population coverage can be computed by,
\begin{equation}
    PC(P) = \sum_{i=1}^{n} y_{i} * pw_{i}
    \label{eq:preset-set-coverage}
\end{equation}

If the preset pool $PP$ is a set of all the possible preset sets, our aim is to find the preset set from the pool that maximizes the population coverage.

\begin{equation}
    P_{max} = argmax_{P \in PP} PC(P)
    \label{eq:maximize-coverage}
\end{equation}





==> results.tex <==
% \section{Results}

In this section, we present the population coverage results for different algorithms and the baseline.
Table \ref{tab:greedy-results} shows the comparison between baseline and the proposed algorithm's population coverage.
The proposed algorithm beats the baseline by 17\% to 8 \% as preset number increases from 20 to 40 in increments of 5.

All the developed presets can be seen in PCA plots shown in Figure \ref{fig:greedy-pca-plots}.
It can be concluded from the results that Genetic Algorithm yields the best results in terms of population coverage compared to the other two methods.

% Bullets
% \begin{itemize}
%     \item First compare clustering, genetic algorithm and greedy algorithm's coverage along with their PCA plots
%     \item Next compare subgroup results for Genetic Algorithm along with PCA plots
%     \item Results suggest that Genetic algorithm beats clustering and greedy algorithm by 3.2\% to 0.5 \% as n goes from 20 to 40 with the increments of 5
%     \item Results also suggest that developing presets for subgroup is beneficial and increases coverage upto 10\%.
%     \item Discuss JND plots and see how good or bad presets are generated by each method.
% \end{itemize}

% Data: GA Coverage data
% For n: 20, max: 71.09, min: 63.93
% For n: 25, max: 80.70, min: 74.64
% For n: 30, max: 85.66, min: 80.57
% For n: 35, max: 88.85, min: 85.12
% For n: 40, max: 90.94, min: 87.80
%
% Data: Greedy
% Coverage[20] is: 67.11672
% Coverage[25] is: 78.87016
% Coverage[30] is: 83.70317
% Coverage[35] is: 86.81270
% Coverage[40] is: 88.86443
%
% Data: Clustering
% Coverage is:  53.95680707114804
% Coverage is:  65.3043699563555
% Coverage is:  73.54870808342237
% Coverage is:  76.63277442318926
% Coverage is:  82.3593167757447


We also explored the best performing algorithm (i.e., Genetic Algorithm) on different demographic subsets.
Table \ref{tab:subgroup_coverate_data} and Table \ref{tab:subgroup_coverate_data} show the population coverage results for female; age > 65 and female; age <= 65 subgroup. 
Similarly, Table \ref{tab:subgroup_coverate_data} and Table \ref{tab:subgroup_coverate_data} show the population coverage results for male; age > 65 and male; age <= 65 subgroup.
In these results, the first column represents the total population coverage by generic GA presets (derived by using all NHANES data).
The second column represents the subgroup population coverage by generic GA presets.
The third column represents the subgroup population coverage by presets derived from subgroup data only.
We can conclude from the results that presets generated by running the algorithm on subgroups generates better population coverage than generic presets.
% Figure \ref{fig:female-pca-plots} and Figure \ref{fig:male-pca-plots} shows the representation of generated presets by different techniques for different subgroups.



\begin{figure*} % for sub figures over two columns in 
\centering
\subfloat[20 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/greedy_results/20_greedy_presets_PCA.png}}
\hfil
% \subfloat[25 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/greedy_results/25_greedy_presets_PCA.png}}
\hfil
\subfloat[30 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/greedy_results/30_greedy_presets_PCA.png}}
\hfil
% \subfloat[35 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/greedy_results/35_greedy_presets_PCA.png}}
\hfil
\subfloat[40 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/greedy_results/40_greedy_presets_PCA.png}}
\caption{Representation of Presets in PCA space. (GA Presets, Greeedy Presets and Clustering presets)}
\label{fig:greedy-pca-plots}
\end{figure*}

% \Figure[b](topskip=0pt, botskip=0pt, midskip=0pt){
% Figures/PCA_Results_Plots/age_results/20_presets_gt_lt_PCA.png}
% {20 presets. \label{fig:presets-20}}

% \begin{figure*} % for sub figures over two columns in 
% \centering
% \subfloat[20 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/age_results/20_presets_gt_lt_PCA.png}}
% \hfil
% \subfloat[25 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/age_results/25_presets_gt_lt_PCA.png}}
% \hfil
% \subfloat[30 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/age_results/30_presets_gt_lt_PCA.png}}
% \hfil
% \subfloat[35 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/age_results/35_presets_gt_lt_PCA.png}}
% \hfil
% \subfloat[40 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/age_results/40_presets_gt_lt_PCA.png}}
% \caption{Age > 65 / Age <= 65 PCA Plots}
% \label{fig:age-pca-plots}
% \end{figure*}

% \begin{figure*} % for sub figures over two columns in 
% \centering
% \subfloat[20 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/m_f_results/20_presets_PCA.png}}
% \hfil
% \subfloat[25 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/m_f_results/25_presets_PCA.png}}
% \hfil
% \subfloat[30 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/m_f_results/30_presets_PCA.png}}
% \hfil
% \subfloat[35 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/m_f_results/35_presets_PCA.png}}
% \hfil
% \subfloat[40 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/m_f_results/35_presets_PCA.png}}
% \caption{Gender PCA Plots}
% \label{fig:gender-pca-plots}
% \end{figure*}



% \begin{table}[h]
% \caption{Population coverage results for (female, age > 65) subgroup}
% \label{tab:female-results-age-gt-65}
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{|p{54pt}|p{54pt}|p{54pt}|p{54pt}|}
% \hline
% Preset number & GA Combined Population Presets & GA Combined Population Presets (Female; age > 65 coverage) & GA Female; age > 65 subgroup Presets \\
%  \hline\hline
%  20 & 0.710 & 0.805 & \textbf{0.821} \\
%  \hline
%  25 & 0.807 & 0.890 & \textbf{0.894} \\
%  \hline
%  30 & 0.856 & 0.920 & \textbf{0.931} \\
%  \hline
%  35 & 0.888 & 0.945 & \textbf{0.950} \\
%  \hline
%  40 & 0.909 & 0.953 & \textbf{0.957} \\
% \hline
% \end{tabular}
% \end{table}

% example of two column table

\begin{table*}[t]
\caption{Population coverage results for specific subgroup presets}
  \centering
  \begin{tabular}{||p{37pt}|p{37pt}||p{37pt}|p{37pt}||p{37pt}|p{37pt}||p{37pt}|p{37pt}||p{37pt}|p{37pt}||}
  \hline
Preset number & GA Combined Population Presets & GA Combined Population Presets (Female; age > 65 coverage) & GA Female; age > 65 subgroup Presets & GA Combined Population Presets (Female; age <= 65 coverage) & GA Female; age <= 65 subgroup Presets
& GA Combined Population Presets (Male; age > 65 coverage) & GA Male; age > 65 subgroup Presets & GA Combined Population Presets (Male; age <= 65 coverage) & GA Male; age <= 65 subgroup Presets  \\
 \hline\hline
%     10 & 0.326 & ?? & ?? & ?? & ?? & ?? & ?? & ?? & ??\\
%   \hline
%     15 & 0.558 & ?? & ?? & ?? & ?? & ?? & ?? & ?? & ??\\
%   \hline
    20 & 0.710 & 0.805 & \textbf{0.821} & 0.753 & \textbf{0.833} & 0.628 & \textbf{0.720} & 0.624 & \textbf{0.710}\\
  \hline
    25 & 0.807 & 0.890 & \textbf{0.894} & 0.826 & \textbf{0.867} & 0.738 & \textbf{0.802} & 0.743 & \textbf{0.797}\\
  \hline
   30 & 0.856 & 0.920 & \textbf{0.931} & 0.876 & \textbf{0.904} & 0.798 & \textbf{0.860} & 0.807 & \textbf{0.851}\\
  \hline
   35 & 0.888 & 0.945 & \textbf{0.950} & 0.919 & \textbf{0.936} & 0.834 & \textbf{0.901} & 0.834 & \textbf{0.876}\\
  \hline
   40 & 0.909 & 0.953 & \textbf{0.957} & 0.940 & \textbf{0.951} & 0.867 & \textbf{0.910} & 0.863 & \textbf{0.900}\\
  \hline
  \end{tabular}
  \label{tab:subgroup_coverate_data}
\end{table*}

Table \ref{tab:variations-effects} shows the population coverage by GA generated presets while using different data to generate variation weights.
Center columns shows the deviations in coverage when using bootstrap data to compute the population coverage.
Right column shows the population coverage when using the non-centered data for weight compuation.
These results show that generated presets are robust enough to capture similar population coverage given the underlying distribution of the data remains the same.
Further, if data changes significantly, population coverage will take a significant hit when $n=20$ but different seems to be lowering down as we increase n from 20 to 40.

% \begin{table}[h]
% \caption{Population coverage results for (female, age <= 65) subgroup}
% \label{tab:female-results-age-lt-65}
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{|p{54pt}|p{54pt}|p{54pt}|p{54pt}|}
% \hline
% Preset number & GA Combined Population Presets & GA Combined Population Presets (Female; age <= 65 coverage) & GA Female; age <= 65 subgroup Presets\\
%  \hline\hline
%  20 & 0.710 & 0.753 & \textbf{0.833} \\
%  \hline
%  25 & 0.807 & 0.826 & \textbf{0.867} \\
%  \hline
%  30 & 0.856 & 0.876 & \textbf{0.904} \\
%  \hline
%  35 & 0.888 & 0.919 & \textbf{0.936} \\
%  \hline
%  40 & 0.909 & 0.940 & \textbf{0.951} \\
% \hline
% \end{tabular}
% \label{tab1}
% \end{table}

% \begin{figure*} % for sub figures over two columns in 
% \centering
% \subfloat[20 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/female_results/20_presets_female_gt_lt_PCA.png}}
% \hfil
% \subfloat[25 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/female_results/25_presets_female_gt_lt_PCA.png}}
% \hfil
% \subfloat[30 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/female_results/30_presets_female_gt_lt_PCA.png}}
% \hfil
% \subfloat[35 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/female_results/35_presets_female_gt_lt_PCA.png}}
% \hfil
% \subfloat[40 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/female_results/40_presets_female_gt_lt_PCA.png}}
% \caption{{Representation of Presets in PCA space. (GA Presets for overall population and female subgroup)}}
% \label{fig:female-pca-plots}
% \end{figure*}

% \begin{table}[h]
% \caption{Population coverage result for male; age > 65 subgroup}
% \label{tab:male-results-age-gt-65}
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{|p{54pt}|p{54pt}|p{54pt}|p{54pt}|}
% \hline
% Preset number & GA Combined Population Presets & GA Combined Population Presets (Male; age > 65 coverage) & GA Male; age > 65 subgroup Presets\\
%  \hline\hline
%  20 & 0.710 & 0.628 & \textbf{0.720} \\
%  \hline
%  25 & 0.807 & 0.738 & \textbf{0.802} \\
%  \hline
%  30 & 0.856 & 0.798 & \textbf{0.860} \\
%  \hline
%  35 & 0.888 & 0.834 & \textbf{0.901} \\
%  \hline
%  40 & 0.909 & 0.867 & \textbf{0.910} \\
% \hline
% \end{tabular}
% \end{table}

% \begin{table}[h]
% \caption{Population coverage result for male; age <= 65 subgroup}
% \label{tab:male-results-age-lt-65}
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{|p{54pt}|p{54pt}|p{54pt}|p{54pt}|}
% \hline
% Preset number & GA Combined Population Presets & GA Combined Population Presets (Male; age <= 65 coverage) & GA Male; age <= 65 subgroup Presets \\
%  \hline\hline
%  20 & 0.710 & 0.624 & \textbf{0.710} \\
%  \hline
%  25 & 0.807 & 0.743 & \textbf{0.797} \\
%  \hline
%  30 & 0.856 & 0.807 & \textbf{0.851} \\
%  \hline
%  35 & 0.888 & 0.834 & \textbf{0.876} \\
%  \hline
%  40 & 0.909 & 0.863 & \textbf{0.900} \\
% \hline
% \end{tabular}
% \end{table}




\begin{table}[h]
\caption{Population coverage deviations}
\label{tab:variations-effects}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|p{54pt}|p{54pt}|p{54pt}|p{54pt}|}
\hline
Preset number & GA Combined Population Presets & GA Combined Population Presets (Bootstrap data) & GA Combined Population Presets (Non-Centered data)\\
 \hline\hline
 20 & 0.710 & 0.710 (± 0.008) & 0.635 \\
 \hline
 25 & 0.807 & 0.807 (± 0.006) & 0.776 \\
 \hline
 30 & 0.856 & 0.856 (± 0.004) & 0.825 \\
 \hline
 35 & 0.888 & 0.888 (± 0.003) & 0.857 \\
 \hline
 40 & 0.909 & 0.909 (± 0.004) & 0.884 \\
\hline
\end{tabular}
\end{table}

% \begin{figure*} % for sub figures over two columns in 
% \centering
% \subfloat[20 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/male_results/20_presets_male_gt_lt_PCA.png}}
% \hfil
% \subfloat[25 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/male_results/25_presets_male_gt_lt_PCA.png}}
% \hfil
% \subfloat[30 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/male_results/30_presets_male_gt_lt_PCA.png}}
% \hfil
% \subfloat[35 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/male_results/35_presets_male_gt_lt_PCA.png}}
% \hfil
% \subfloat[40 Presets]{\includegraphics[width=0.32\linewidth]{Figures/PCA_Results_Plots/male_results/40_presets_male_gt_lt_PCA.png}}
% \caption{Representation of Presets in PCA space. (GA Presets for overall population and male subgroup)}
% \label{fig:male-pca-plots}
% \end{figure*}

% \begin{figure}[b]
%      \centering
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/PCA_Results_Plots/age_results/20_presets_gt_lt_PCA.png}
%          \caption{$y=x$}
%          \label{fig:y equals x}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/PCA_Results_Plots/age_results/25_presets_gt_lt_PCA.png}
%          \caption{$y=3sinx$}
%          \label{fig:three sin x}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/PCA_Results_Plots/age_results/30_presets_gt_lt_PCA.png}
%          \caption{$y=5/x$}
%          \label{fig:five over x}
%      \end{subfigure}
%         \caption{Three simple graphs}
%         \label{fig:three graphs}
% \end{figure}




% \begin{table}[h]
% \caption{Greedy Algorithm Results}
% \label{tab:greedy-results}
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{|p{42pt}|p{42pt}|p{42pt}|p{42pt}|p{42pt}|}
% \hline
% Cluster number & Genetic Algorithm (Combined) & Greedy Algorithm & Greedy Algorithm (With weights) & Clustering (Combined) \\
%  \hline\hline
%  20 & \textbf{0.681} & 0.615 & 0.649 & 0.530 \\
%  \hline
%  25 & \textbf{0.785} & 0.718 & 0.752 & 0.671 \\
%  \hline
%  30 & \textbf{0.835} & 0.782 & 0.818 & 0.749 \\
%  \hline
%  35 & \textbf{0.869} & 0.831 & 0.857 & 0.819 \\
%  \hline
%  40 & \textbf{0.891} & 0.872 & 0.886 & 0.862 \\
% \hline
% \end{tabular}
% \label{tab1}
% \end{table}






